Learning-Based Dimensionality Reduction for Computing Compact and Effective Local Feature Descriptors

A distinctive representation of image patches in form of features is a key component of many computer vision and robotics tasks, such as image matching, image retrieval, and visual localization. State-of-the-art descriptors, from hand-crafted descriptors such as SIFT to learned ones such as HardNet, are usually high dimensional; 128 dimensions or even more. The higher the dimensionality, the larger the memory consumption and computational time for approaches using such descriptors. In this paper, we investigate multi-layer perceptrons (MLPs) to extract low-dimensional but high-quality descriptors. We thoroughly analyze our method in unsupervised, self-supervised, and supervised settings, and evaluate the dimensionality reduction results on four representative descriptors. We consider different applications, including visual localization, patch verification, image matching and retrieval. The experiments show that our lightweight MLPs achieve better dimensionality reduction than PCA. The lower-dimensional descriptors generated by our approach outperform the original higher-dimensional descriptors in downstream tasks, especially for the hand-crafted ones. The code will be available at https://github.com/PRBonn/descriptor-dr.

==> stachnisslab-math.tex <==
%% Math definitions used at the Stachniss-Lab

% argmax operator
\def\argmax{\mathop{\rm argmax}}

% argmain operator
\def\argmin{\mathop{\rm argmin}}

%% Spaces
\newcommand{\PP}{\mathbb{P}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\ZZ}{\mathbb{Z}}

% O-Notation
\newcommand{\bigO}[1]{$\mathcal{O}(#1)$}

% absolute value
\newcommand{\abs}[1]{|#1|}

% Norm
\newcommand{\norm}[1]{\lVert#1\lVert}

% 1/2 as math
\newcommand{\half}{\frac{1}{2}}

% sign 
\newcommand{\sign}[0]{{\mbox{sign}}}

% specif matrix dimensions under a matrix
\newcommand{\mdim}[3]{\stackrel[\mbox{\tiny $#2\!\!\times\!\!#3$}]{}{#1}}

% math boldface #1  
\renewcommand{\b}[1]{\mbox{\boldmath$#1$}}

% =\b (for compatability)
\renewcommand{\d}[1]{\b {#1}}

% vector
\renewcommand{\v}[1]{{\b #1}} 

% matrix
\newcommand{\m}[1]{{\mbox{{\sffamily\slshape{#1\/}}}}}

% homogeneous vector
\newcommand{\q}[1]{{{\bf #1}}}

% homogeneous matrix
\newcommand{\mq}[1]{{\mbox{{\sffamily{#1}}}}}

% transpose vector or matrix
\newcommand{\tr}[0]{\sf T}              % transpose without ^  
\newcommand{\trans}[0]{^\tr}            % normal
\newcommand{\transs}[0]{{'}^\tr}        % ‘ trans
\newcommand{\transss}[0]{{''}^\tr}      % ‘‘ trans
\newcommand{\transsss}[0]{{'''}^\tr}    % ’’’ trans
\newcommand{\transi}[0]{^{-\tr}}        % - trans
\newcommand{\transa}[0]{^{*\tr}}        % * trans

%inverse 
\newcommand{\inv}{^{-1}}

% Differential operator d
\newcommand{\diff}[0]{\mbox{d}}

% degree
\newcommand{\degrees}{{\mbox{$^\circ$}}}

% Diag 
\newcommand{\Diag}[0]{{\mbox{Diag}}}

% trace  
\newcommand{\trace}[0]{{\mbox{tr}\,}}

% rank 
\newcommand{\rank}[0]{{\mbox{rank}\,}}

% nullspace 
\newcommand{\nullspace}[0]{{\mbox{null}}}

%atan2 (use with one argument: sin- and cos-part  seperated by , or ;)
\newcommand{\atan}[1]{\mbox{atan2} \, ({#1})}

%acot2 (use with one argument: sin- and cos-part  seperated by , or ;)
\newcommand{\acot}[1]{\mbox{acot2} \, ({#1})}

% specify coordinate system of an element
%#1 = system, #2 = variable
\newcommand{\cs}[2]{\; ^{#1}\!\,{\mbox{#2}}}

% specify coordinate system of matrix from to
% #1 = variable, #2 = from, #3 = to,
\newcommand{\cft}[3]{\; ^{#1}\!\,{\mbox{#2}}_{#3}}

%Rotationmatrix with index and angle: R_i(a)%
\newcommand{\rot}[2]{\m{R}_{#1}(#2)}

%Rotationmatrix transposed with index and angle:  R^T_i(a)%
\newcommand{\rott}[2]{\m{R}\trans_{#1}(#2)}

% Jacobian
\newcommand{\J}{\m J} 


%2 vector%
\newcommand{\zvector}[2]
  {    \left[
          \begin{array}{c}
            {#1} \\ {#2}
        \end{array}
       \right] }

%3 vector%
\newcommand{\dvector}[3]
  {    \left[
          \begin{array}{c}
            {#1} \\ {#2} \\{#3}
        \end{array}
       \right] }

%4 vector%
\newcommand{\vvector}[4]
  {    \left[
          \begin{array}{c}
            {#1} \\ {#2} \\{#3} \\ {#4}
          \end{array}
       \right] }

%5 vector%
\newcommand{\fvector}[5]
  {    \left[
          \begin{array}{c}
            {#1} \\ {#2} \\{#3} \\ {#4}\\ {#5}
          \end{array}
       \right] }

%%6 vector%
\newcommand{\svector}[6]
  {    \left[
          \begin{array}{c}
            {#1} \\ {#2} \\{#3} \\ {#4}\\ {#5}\\ {#6}
          \end{array}
       \right] }

%%7 vector%
\newcommand{\sivector}[7]
  {    \left[
          \begin{array}{c}
            {#1} \\ {#2} \\{#3} \\ {#4}\\ {#5}\\ {#6}\\ {#7}
          \end{array}
       \right] }

%%8 vector%
\newcommand{\avector}[8]
  {    \left[
          \begin{array}{c}
            {#1} \\ {#2} \\{#3} \\ {#4}\\ {#5}\\ {#6}\\ {#7}\\ {#8}
          \end{array}
       \right] }
       
%%9 vector%
\newcommand{\nvector}[9]
  {    \left[
          \begin{array}{c}
            {#1} \\ {#2} \\{#3} \\ {#4}\\ {#5}\\ {#6}\\ {#7}\\ {#8}\\ {#9}
          \end{array}
       \right] }


%2 vector transposed%
\newcommand{\zvectort}[2]
  {    \left[
            {#1} \; {#2}
       \right] }


%3 vector transposed%
\newcommand{\dvectort}[3]
  {    \left[
            {#1} \; {#2}\; {#3}
       \right] }

%4 vector transposed%
\newcommand{\vvectort}[4]
  {    \left[
            {#1} \; {#2}\; {#3}\; {#4}
       \right] }


%2 x 3 matrix%
\newcommand{\zdmatrix}[6]
  {    \left[
          \begin{array}{ccc}
            {#1} & {#2} & {#3} \\
            {#4} & {#5} & {#6} 
          \end{array}
       \right] }

%2 x 4 matrix%
\newcommand{\zvmatrix}[8]
  {    \left[
          \begin{array}{cccc}
            {#1} & {#2} & {#3} & {#4}\\
            {#5} & {#6} & {#7} & {#8}
          \end{array}
       \right] }
%4 x 2 matrix%
\newcommand{\vzmatrix}[8]
  {    \left[
          \begin{array}{cc}
            {#1} & {#2} \\ {#3} & {#4}\\
            {#5} & {#6} \\ {#7} & {#8}
          \end{array}
       \right] }

%3 x 2 matrix%
\newcommand{\dzmatrix}[6]
  {    \left[
          \begin{array}{ccc}
            {#1} & {#2} \\
            {#3} & {#4} \\
            {#5} & {#6}
          \end{array}
       \right] }
%

%2 x 2 matrix%
\newcommand{\zmatrix}[4]
  {    \left[
          \begin{array}{cc}
            {#1} & {#2} \\
            {#3} & {#4}
          \end{array}
       \right] }

%3 x 3 matrix%
\newcommand{\dmatrix}[9]
  {    \left[
          \begin{array}{ccc}
            {#1} & {#2} & {#3} \\
            {#4} & {#5} & {#6} \\
            {#7} & {#8} & {#9}
          \end{array}
       \right] }

%4 x 4 matrix%
%% not allowed, max 9 parameters!

%Determinant 2x2
\newcommand{\zdet}[4]
  {    \left|
          \begin{array}{cc}
            {#1} & {#2} \\
            {#3} & {#4}
          \end{array}
       \right| }

%Determinant 3x3
\newcommand{\ddet}[9]
  {    \left|
          \begin{array}{ccc}
            {#1} & {#2} & {#3}\\
            {#4} & {#5} & {#6}\\
            {#7} & {#8} & {#9}
          \end{array}
       \right| }


 
% General matrix: #1: #colums, #2: String for elemets
% incl. //
\newcommand{\matr}[2]{%
\left[ \begin{array}{*#1{c} }    #2   \end{array} \right] %
  }

 % General Determinant:  #1: #colums, #2: String for elemets
% incl. //
\newcommand{\dete}[2]{%
\left| \begin{array}{*#1{c}}    #2   \end{array} \right| %
  }

 % Boldface abbrevs
\newcommand{\bA}{\b A}
\newcommand{\bB}{\b B}
\newcommand{\bC}{\b C}
\newcommand{\bD}{\b D}
\newcommand{\bE}{\b E}
\newcommand{\bF}{\b F}
\newcommand{\bG}{\b G}
\newcommand{\bH}{\b H}
\newcommand{\bI}{\b I}
\newcommand{\bJ}{\b J}
\newcommand{\bK}{\b K}
\newcommand{\bL}{\b L}
\newcommand{\bM}{\b M}
\newcommand{\bN}{\b N}
\newcommand{\bO}{\b O}
\newcommand{\bP}{\b P}
\newcommand{\bQ}{\b Q}
\newcommand{\bR}{\b R}
\newcommand{\bS}{\b S}
\newcommand{\bT}{\b T}
\newcommand{\bU}{\b U}
\newcommand{\bV}{\b V}
\newcommand{\bW}{\b W}
\newcommand{\bX}{\b X}
\newcommand{\bY}{\b Y}
\newcommand{\bZ}{\b Z}

\newcommand{\ba}{\b a}
\newcommand{\bb}{\b b}
\newcommand{\bc}{\b c}
\newcommand{\bd}{\b d}
\newcommand{\be}{\b e}
%\newcommand{\bf}{\b f}
\newcommand{\bg}{\b g}
\newcommand{\bh}{\b h}
\newcommand{\bi}{\b i}
\newcommand{\bj}{\b j}
\newcommand{\bk}{\b k}
\newcommand{\bl}{\b l}
\newcommand{\bm}{\b m}
\newcommand{\bn}{\b n}
\newcommand{\bo}{\b o}
\newcommand{\bp}{\b p}
\newcommand{\bq}{\b q}
\newcommand{\br}{\b r}
\newcommand{\bs}{\b s}
\newcommand{\bt}{\b t}
\newcommand{\bu}{\b u}
\newcommand{\bv}{\b v}
\newcommand{\bw}{\b w}
\newcommand{\bx}{\b x}
\newcommand{\by}{\b y}
\newcommand{\bz}{\b z}

\newcommand{\dA}{\b A}
\newcommand{\dB}{\b B}
\newcommand{\dC}{\b C}
\newcommand{\dD}{\b D}
\newcommand{\dF}{\b F}
\newcommand{\dG}{\b G}
\newcommand{\dH}{\b H}
\newcommand{\dI}{\b I}
\newcommand{\dJ}{\b J}
\newcommand{\dK}{\b K}
\newcommand{\dL}{\b L}
\newcommand{\dM}{\b M}
\newcommand{\dN}{\b N}
\newcommand{\dO}{\b O}
\newcommand{\dP}{\b P}
\newcommand{\dQ}{\b Q}
\newcommand{\dR}{\b R}
\newcommand{\dS}{\b S}
\newcommand{\dT}{\b T}
\newcommand{\dU}{\b U}
\newcommand{\dV}{\b V}
\newcommand{\dW}{\b W}
\newcommand{\dX}{\b X}
\newcommand{\dY}{\b Y}
\newcommand{\dZ}{\b Z}

\newcommand{\mA}{\m A}
\newcommand{\mB}{\m B}
\newcommand{\mC}{\m C}
\newcommand{\mD}{\m D}
\newcommand{\mF}{\m F}
\newcommand{\mG}{\m G}
\newcommand{\mH}{\m L}
\newcommand{\mI}{\m I}
\newcommand{\mJ}{\m J}
\newcommand{\mK}{\m K}
\newcommand{\mL}{\m L}
\newcommand{\mM}{\m M}
\newcommand{\mN}{\m N}
\newcommand{\mO}{\m O}
\newcommand{\mP}{\m P}
\newcommand{\mQ}{\m Q}
\newcommand{\mR}{\m R}
\newcommand{\mS}{\m S}
\newcommand{\mT}{\m T}
\newcommand{\mU}{\m U}
\newcommand{\mV}{\m V}
\newcommand{\mW}{\m W}
\newcommand{\mX}{\m X}
\newcommand{\mY}{\m Y}
\newcommand{\mZ}{\m Z}



==> tables/veri_results_HardNet.tex <==
\begin{tabular}{@{}lcccccccc@{}} 
\toprule
Training  & Notredame & Yosemite & Liberty  & Yosemite & Liberty & Notredame  & Mean    \\
\cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7} 
Test    & \multicolumn{2}{c}{Liberty} & \multicolumn{2}{c}{Notredame} & \multicolumn{2}{c}{Yosemite} & FPR \\
\cmidrule(r){1-8}
%\multicolumn{8}{c}{No augmentation} \\
%\cmidrule(r){1-8}
HardNet     & 2.28     & 3.25         & \hlf{0.57}      &  \hlf{0.96}     & \hlf{2.13}     & \hlf{2.22}    & 1.90         \\ \hline

HardNet-PCA-16 & \hls{9.84}     & 16.57         & \hls{6.74}       &  13.66     & \hls{15.82}     &\hls{14.46}    & \hls{12.84} \\
HardNet-AE-16  & 13.13     & 20.57         & 9.79       &  17.0     & 19.98     & 18.0    & 16.41   \\
HardNet-SS-16 & 11.75 &15.67 &9.73 &\hls{11.62} & 17.06 &16.91 &13.79\\
HardNet-Triplet-16   & 11.45     & \hls{15.27}       & 7.35         & 13.69   & 17.28     & 17.38     & 13.73  \\ \hline

HardNet-PCA-24          & \hls{5.23} & 9.26    & \hls{3.40}     & \hls{6.39}     & \hls{9.17}     & \hls{8.45}     &\hls{6.98} \\
HardNet-AE-24          & 6.38 & 9.21    & 4.70    & 7.02     & 11.52     & 10.47    & 8.21 \\
HardNet-SS-24 & 6.30 &8.93 &5.55 &7.35 & 10.81 &10.61 &8.25\\
HardNet-Triplet-24   & 5.95     &\hls{8.44}        & 4.06         &6.70     & 9.96     & 10.25    & 7.56  \\ \hline

HardNet-PCA-32 & \hls{3.16}     & 5.68         & \hls{2.02}       &  3.63     & \hls{6.22}     & \hls{5.79}     & \hls{4.41} \\
HardNet-AE-32  & 3.65     & \hls{5.34}         & 2.69       &  \hls{3.58}     & 7.43     & 6.88    & 4.92   \\
HardNet-SS-32 & 3.98 &5.99 &3.78 &4.98& 8.14 &7.74 &5.76\\
HardNet-Triplet-32   & 3.58     & 5.42        & 2.44         & 4.40     & 7.13     & 7.34     & 5.05  \\ \hline

HardNet-PCA-64 & \hlf{0.85}     & 1.63         & \hls{0.78}      &  1.11     & 2.73     & \hls{2.41}     & 1.58 \\
HardNet-AE-64  & 0.89     & \hlf{1.27}         & \hls{0.78}       &  \hlf{0.96}     & \hls{2.70}     & 2.71    & \hlf{1.55}   \\
HardNet-SS-64 & 1.50 &2.30 & 1.41 &2.27& 3.67  &3.57 &2.45\\
HardNet-Triplet-64   & 1.02     & 1.53        & 0.85         & 1.12     & 2.85     & 3.12     &1.74  \\

\bottomrule
\end{tabular}

==> tables/veri_results_MKD.tex <==
\begin{tabular}{@{}lcccccccc@{}} 
\toprule
Training  & Notredame & Yosemite & Liberty  & Yosemite & Liberty & Notredame  & Mean    \\
\cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7} 
Test    & \multicolumn{2}{c}{Liberty} & \multicolumn{2}{c}{Notredame} & \multicolumn{2}{c}{Yosemite} & FPR \\
\cmidrule(r){1-8}
%\multicolumn{8}{c}{No augmentation} \\
%\cmidrule(r){1-8}
MKD     & \multicolumn{2}{c}{12.55}  & \multicolumn{2}{c}{5.24}   & \multicolumn{2}{c}{8.01}  & 8.60         \\ \hline

MKD-PCA-16 &28.74     & 34.17         & 15.44       &  20.74     & 23.45     & 23.56     & 24.35 \\
MKD-AE-16  &34.15     & 40.96         &20.12       &  26.38     & 31.61     & 31.73    &30.82   \\
MKD-SS-16 & 26.45 &28.0 &14.90 &15.03&22.20 &21.61 &21.36\\
MKD-Triplet-16   & \hls{15.14}     & \hls{18.50}      & \hls{8.04}         & \hls{9.81}    & \hls{14.56}    & \hls{14.37}     & \hls{13.40} \\ \hline

MKD-PCA-24          & 24.50 & 28.81    & 11.97     & 14.79     & 18.41     & 19.18     &19.61 \\
MKD-AE-24          & 24.16 & 29.95    & 11.49     & 15.94    & 19.76     & 19.67   & 20.16 \\
MKD-SS-24 & 20.67 &20.52 &10.12 &10.29 & 15.18 &14.53 &15.21\\
MKD-Triplet-24   & \hls{11.03}    & \hls{13.58}      & \hls{5.04}        & \hls{6.36}    & \hls{10.13}     & \hls{9.35}     &\hls{9.24}  \\ \hline

MKD-PCA-32 & 21.21    & 26.31         & 9.50       &  12.38     & 15.86     & 15.72     & 16.83 \\
MKD-AE-32  & 19.89     & 24.27         & 8.52       &  12.28     & 14.27     & 14.93    & 15.69   \\
MKD-SS-32 & 16.67 &18.35 &8.09 &8.30& 13.0 &11.65 &12.67\\
MKD-Triplet-32   &\hls{9.30}    &\hls{11.11}       & \hls{3.85}         & \hls{4.73}     & \hls{8.08}    & \hls{7.25}     &\hls{7.38}  \\ \hline

MKD-PCA-64 & 16.15     & 18.05         & 6.58       &  7.46     & 10.96     & 10.52     & 11.62 \\
MKD-AE-64  &14.44     & 16.29        &5.65       & 6.98     &8.99     & 9.57    & 10.32   \\
MKD-SS-64 & 16.12 &16.32 &6.06 &6.83 & 9.86 &9.52 &10.78\\
MKD-Triplet-64   & \hlf{6.88}     & \hlf{7.84}        &\hlf{2.60}         & \hlf{2.89}    & \hlf{5.58}    & \hlf{5.28}    &\hlf{5.17}  \\

\bottomrule
\end{tabular}

==> tables/veri_results_SIFT.tex <==
\begin{tabular}{@{}lcccccccc@{}} 
\toprule
Training  & Notredame & Yosemite & Liberty  & Yosemite & Liberty & Notredame  & Mean    \\
\cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7} 
Test    & \multicolumn{2}{c}{Liberty} & \multicolumn{2}{c}{Notredame} & \multicolumn{2}{c}{Yosemite} & FPR \\
\cmidrule(r){1-8}
%\multicolumn{8}{c}{No augmentation} \\
%\cmidrule(r){1-8}
SIFT     & \multicolumn{2}{c}{31.70}  & \multicolumn{2}{c}{28.04}   & \multicolumn{2}{c}{32.95}  & 30.89         \\ \hline

SIFT-PCA-16 & 27.71     & 30.21         & 23.28       &  23.44     & 27.35     & 24.74     & 26.12 \\
SIFT-AE-16  &28.92     & 32.97         & 23.12       &  25.99     & 30.30     & 27.88   & 28.19   \\
SIFT-SS-16 &28.68 &34.67 &19.72 &20.12 & 25.29 &24.14 &25.43\\
SIFT-Triplet-16   & \hls{19.43}     & \hls{24.55}        & \hls{10.77}        & \hls{14.06}     & \hls{18.31}     & \hls{17.58}    & \hls{17.45}  \\ \hline

SIFT-PCA-24          & 24.36 & 27.43    & 18.32     & 19.32     & 22.54     & 20.58    &22.09 \\
SIFT-AE-24          & 24.03 & 27.62    & 18.34     & 19.53    & 25.37     & 22.43    & 22.88 \\
SIFT-SS-24 & 25.37 &29.65 &15.09 &16.98& 20.89 &19.16 &21.19\\
SIFT-Triplet-24   & \hls{16.31}     &\hls{20.21}       &\hls{7.82}         & \hls{9.75}    & \hls{13.90}     & \hls{12.96}     & \hls{13.49}  \\ \hline

SIFT-PCA-32 & 23.82     & 25.90         & 16.63       &  17.43     & 21.22     & 19.47     & 20.74 \\
SIFT-AE-32  & 22.30    & 24.26         & 16.50       &  17.22     & 22.64     & 21.14    & 20.67   \\
SIFT-SS-32 & 26.61 &25.47 &14.46 &15.10& 18.80 &16.88 &19.55\\
SIFT-Triplet-32   & \hls{14.66}     & \hls{17.62}        & \hls{6.57}         & \hls{7.50}     & \hls{12.15}     & \hls{10.55}    &\hls{11.50}   \\ \hline

SIFT-PCA-64 & 22.22     & 23.63         & 15.23       &  15.43    & 18.24     & 16.81     & 18.59 \\
SIFT-AE-64  & 21.16     & 24.81         & 16.26       &  19.34     & 22.19     &19.46    & 20.53   \\
SIFT-SS-64 &25.70 &24.59 &14.91 &14.76 & 15.89 &15.56 &18.56\\
SIFT-Triplet-64   &\hlf{12.66}      & \hlf{13.50}         & \hlf{5.09}          & \hlf{6.16}     & \hlf{10.16}      & \hlf{9.36}     & \hlf{9.48}  \\

\bottomrule
\end{tabular}

==> tables/veri_results_TFeat.tex <==
\begin{tabular}{@{}lcccccccc@{}} 
\toprule
Training  & Notredame & Yosemite & Liberty  & Yosemite & Liberty & Notredame  & Mean    \\
\cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7} 
Test    & \multicolumn{2}{c}{Liberty} & \multicolumn{2}{c}{Notredame} & \multicolumn{2}{c}{Yosemite} & FPR \\
\cmidrule(r){1-8}
%\multicolumn{8}{c}{No augmentation} \\
%\cmidrule(r){1-8}
TFeat     & 7.39     & 10.31         & 3.06      &  3.80     & 8.06     & \hlf{7.24}     & 6.64         \\ \hline

TFeat-PCA-16 & \hls{6.33}     & 10.52         & \hls{6.77}       &  9.85     & 19.70     & \hls{14.42}     & \hls{11.26}  \\
TFeat-AE-16  & 7.81     & \hls{10.50}         & 7.41       &  \hls{9.77}     &21.40     & 18.76    & 12.60   \\
TFeat-SS-16 & 8.71 &\hls{10.50} &11.18 &10.88 & 19.62 &18.64 &13.25\\
TFeat-Triplet-16   & 10.18     & 13.22       & 9.16        & 12.41    & \hls{18.08}     &16.54     & 13.26 \\ \hline

TFeat-PCA-24          & 4.18 & 7.35    & 4.43     & 6.66     &13.79     & \hls{10.42}     &7.80 \\
TFeat-AE-24          &\hls{3.92} & \hls{5.52}    & \hls{4.31}     & \hls{5.13}     & 14.51     &10.79    & \hls{7.36}  \\
TFeat-SS-24 & 6.88 &7.53 &9.01 &7.93 & 15.0 &13.94 &10.04\\
TFeat-Triplet-24   &5.36     & 7.57        & 5.31         & 6.85     &\hls{12.65}     & 11.48    & 8.20  \\ \hline

TFeat-PCA-32 & 3.61     & 5.99         & 3.60       &  5.49    & 11.92     & 8.64     & 6.54 \\
TFeat-AE-32  & \hls{2.98}     & \hls{3.60}         & \hls{3.21}       &  \hls{3.57}     & 11.38     & \hls{8.38}   & \hls{5.52}    \\
TFeat-SS-32 & 5.36 &6.50 &7.06 &6.77& 12.57 &11.91 &8.36\\
TFeat-Triplet-32   & 4.01     & 4.99        & 4.46        & 4.83     &\hls{10.57}     & 9.45     & 6.38  \\ \hline

TFeat-PCA-64 & 3.12     & 5.70        & 2.98       &  4.70     & 10.23     & \hls{7.36}    & 5.68 \\
TFeat-AE-64  & \hlf{1.87}     & \hlf{2.13}         & \hlf{2.68}       &  \hlf{2.50}     & 8.79     & 7.47    & \hlf{4.24}  \\
TFeat-SS-64 & 3.60 &4.74 &5.48 &5.83&10.98 &9.90 &6.75\\
TFeat-Triplet-64   & 2.40     & 2.94        & 3.41         & 3.37     & \hlf{7.95}     & 7.48     & 4.59  \\

\bottomrule
\end{tabular}
